Mechanistic Understanding and Mitigation of Language Model Non-Factual Hallucinations

State-of-the-art language models (LMs) sometimes generate non-factual hallucinations that misalign with world knowledge. To explore the mechanistic causes of these hallucinations, we create diagnostic datasets with subject-relation queries and adapt interpretability methods to trace hallucinations through internal model representations. We discover two general and distinct mechanistic causes of hallucinations shared across LMs (Llama-2, Pythia, GPT-J): 1) knowledge enrichment hallucinations: insufficient subject attribute knowledge in lower layer MLPs, and 2) answer extraction hallucinations: failure to select the correct object attribute in upper layer attention heads. We also found these two internal mechanistic causes of hallucinations are reflected in external manifestations. Based on insights from our mechanistic analysis, we propose a novel hallucination mitigation method through targeted restoration of the LM's internal fact recall pipeline, demonstrating superior performance compared to baselines.

==> hall-evolution.tex <==
\section{Tracing LM Hallucinations During Pretraining} \label{sec:hall_evol}
We have identified two mechanisms of non-factual hallucinations in LMs. In this section, we design experiments with the goal of understanding how these hallucinations emerge during model pretraining. For example, do early-site and late-site hallucinations exhibit different learning patterns that contribute to their distinctions?  We also aim to explore why the crucial early-site MLP and late-site attention components fail to ``develop'' properly.

\paragraph{Data and models.}
% To study language model hallucinations during pretraining, we evaluate the Pythia-1.4B model suite \cite{biderman2023pythia} on our curated ParaRel factual query dataset. Pythia is a set of pretraining checkpoints for a family of autoregressive LMs trained on public data in the exact same order.  We first take the last checkpoint of Pythia-1.4B and repeat the same evaluation and filtering processes for GPT2-XL on ParaRel dataset described in section \ref{subsec:gpt_cpi} to obtain a dataset of 8,345 queries, where the model hallucinates on 6,664 questions and correctly answers 1,681 of them. Next, we perform causal mediation analysis on hallucinating queries to get average indirect effects for attention heads and MLPs, and categorize the queries into 980 early-site and 5,684 late-site hallucinations. We then evaluate and get intermediate hidden states for all queries on 32 Pythia-1.4B pretraining checkpoints evenly distributed across model learning history.\footnote{See Appendix \ref{appendix:pythia} for details of Pythia evaluation.}  
To study language model hallucinations during pretraining, we evaluate the Pythia model suite \cite{biderman2023pythia} on ParaRel. Pythia is a set of pretraining checkpoints for a family of autoregressive LMs trained on public data in the exact same order. We first take the last checkpoint of Pythia with 1.4 billion parameters and repeat the same evaluation and filtering processes for other LMs on ParaRel dataset described in section \ref{subsec:cpi}, and then perform causal mediation analysis on incorrectly answered queries to get AIEs for attention heads and MLPs, and categorize the queries into early-site and late-site hallucinations based on Equation \ref{eq:rel-ie}. We then evaluate and get intermediate hidden states for all queries on 32 Pythia-1.4B pretraining checkpoints evenly distributed across model learning history.\footnote{See Appendix \ref{appendix:pythia} for details of Pythia evaluation.}  


\paragraph{Development of factual association pipeline.}
We replicate the embedding space projection (ESP) experiments in section \ref{subsec:esp} on Pythia-1.4b checkpoints and compare the results across pretraining steps. For each Pythia-1.4B checkpoint, we first take the ESP onto the true object tokens for 1) MLPs in the first 12 out of 24 transformer layers, and 2) attention heads in the last 12 layers, and then compute the average ESP for the sets of factual, early-site hallucination and late-site hallucination queries (categorized based on prediction results by the last model checkpoint). Figure \ref{fig:pythia_esp} shows the evolution trajectory of true object ESPs on 32 Pythia-1.4b checkpoints. We notice that 1) the learning dynamics of MLPs between late-site hallucination and factual queries are very similar, where they gradually learn to produce positive ESPs to the true object prediction roughly during the first half of pretraining. For early-site hallucinations, the MLPs instead learn to make negative ESPs, again suggesting their lack of true subject knowledge. 2) The upper-layer attentions of Pythia only learn to produce high ESPs for factual queries. Moreover, the attention modules will not learn to distinguish true objects until the early-site MLPs have grown mature ($\sim$70-\textit{th} pretraining step). Taken together, our results suggest that \textit{the early-site MLPs and late-site attentions together form a two-step pipeline of fact recall that emerges progressively during pretraining, and failing to develop either of them will lead to non-factual hallucinations}. 


\begin{figure}[]
\centering
\includegraphics[width=0.9\columnwidth]{figures/pythia-1.4b_esp.pdf}
\caption{Average embedding space projections to the true object tokens for lower-layer MLPs (up) and upper-layer attention modules (down) of Pythia-1.4b pretraining checkpoints. The red vertical line indicates a ``phase change'' when the lower layer MLPs finish their learning, and upper layer attention heads start to develop. }
\label{fig:pythia_esp}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> hall-mechanisms.tex <==
\section{Mechanisms of Hallucinations} \label{sec:hall_mech}

\subsection{Causal tracing of factual errors} \label{subsec:cpi}
\paragraph{Method.} 
The intermediate hidden states $H$ produced by $G$ during model inference form a causal dependency graph \cite{pearl2001direct} that contains many paths from the input sequence to the output (next-token prediction), and we wish to understand if there are specific hidden states that are more important than others when producing a hallucination. This is a natural case for \textit{causal mediation analysis}, which quantifies the contribution of intermediate variables in causal graphs. For more information about causal mediation analysis of language models, see \citet{vig2020investigating}.

We adapt the framework of \citet{meng2022locating} to locate LM components that cause factual errors via the task of factual open-domain questions on structured queries. In particular, given a fact represented as a subject-relation-object triple $(s,r,o)$, we provide an LM $G$ with a query prompt $u$ containing $(s,r)$ (e.g., ``Toulouse is the twin city of \_\_'') with $o$ as a true continuation (e.g., ``Atlanta''). We examine the cases where $G$ predicts an incorrect object $o'$ as the next token(s) given $u$, and aim to locate which intermediate hidden states in the computation graph of $G$ led to the hallucination. We consider $G$ to be a ``corrupted'' model with certain modules failing to compute the ``clean'' representations that could otherwise lead to the correct answer $o$, and measure the contribution of each module through three model runs: 

% a model needs to predict an attribute  of a given subject-relation pair (s, r). 
% the cases where a language model $G$ generates factually incorrect outputs that contradict with world knowledge. Given a subject-relation-object triple $(s,r,o)$, and a query prompt $u$ (e.g., ``The Space Needle is in downtown \_\_'') containing $s,r$ with true next word completion $o$ (e.g., ``Seattle''), we would like to investigate the internal computational patterns of an auto-regressive language model $G$ where it incorrectly predicts another entity $o'$ as a continuation of the prompt $u$ when taking the static token embeddings $E(u)$ as inputs (i.e. $o'$ is a hallucination by $G$ given $u$). 

\begin{enumerate}
    \item In the \textbf{hallucination run}, we pass $u$ into $G$ and extract all intermediate hidden representations $Z$ as defined in Section~\ref{sec:background}, and compute the log likelihood ratio $y = \log\frac{p(o'|E(u))}{p(o|E(u))}$ between the true and hallucinated objects, which quantifies the ``degree of hallucination'' of $G$. For a hallucinating prediction, we would observe $y > 0$.  
    \item In the \textbf{mitigation run}, we follow \citet{meng2022locating} and add a Gaussian noise $\epsilon \sim \mathcal{N}(0, 1)$ to the input token embeddings $E(u)$, so that when taking the intervened $E^*(u)=E(u) + \epsilon$ as inputs, the log-likelihood ratio between the hallucinated and the factual object would decrease 
    (i.e., we only take noises with $y_* = \log\frac{p(o'|E^*(u))}{p(o|E^*(u))} < y$, indicating that the model becomes more ``truthful'' after noise injections). We again extract all intermediate hidden representations, denoted as $Z^*$.
    \item In the \textbf{mitigation-with-hallucination-state run}, we run $G$ on $u$ with perturbed input embeddings $E^*(u)$ as in the mitigation run, and hook $G$ by forcing a particular hidden representation $z^* \in Z^*$ to be the hidden representation $z$ during the hallucination run. We then compute the log likelihood ratio $y_{E^*,z} = \log\frac{p(o'|E^*(u),z)}{p(o|E^*(u),z)}$ to see how it changes compared to step 2. 
    % \item In the \textbf{hallucination-with-mitigation-state run}, we run $G$ on the original prompt $u$ as in the hallucination run, and hook $G$ by forcing a particular hidden representation $z \in Z$ to be the hidden representation $z^*$ during the mitigation run. We then compute the log likelihood ratio $y_{E,z^*} = \log\frac{p(o'|E(u),z^*)}{p(o|E(u),z^*)}$ to see how it changes compared to step 2. 
\end{enumerate}

\begin{figure*}[ht]
\centering
\includegraphics[width=.9\textwidth]{figures/cpi_modules_Llama-2-7b-chat-hf-annotated.pdf}
% \caption{\textbf{Average Indirect Effect (AIE)} of individual model components to non-factual hallucinations over 6,401 ParaRel queries that are incorrectly answered by GPT-2 XL. $\Delta \text{AIE}(y,u)$ is defined as the difference in AIE between 1) the attention outputs of the last 24 transformer layers and 2) the MLP outputs of the first 24 GPT-2 XL layers.}
\caption{\textbf{Average Indirect Effect (AIE)} of hidden representations produced by individual model components to non-factual hallucinations over ParaRel queries that are incorrectly answered by Llama-2-7b-chat. The relative indirect effect metric $\Delta \overline{\text{IE}}(y,u)$ of distinguishing early-site and late-site hallucinations is defined as the difference between the mean AIE of 1) the hidden representations of the last relation token by upper layer attentions/MLPs (blue dashed boxes), and 2) the hidden representations of the first subject token by lower layer attentions/MLPs (red dashed boxes).
}
\label{fig:cpi-modules-Llama}
\end{figure*}

\begin{figure*}[t!]
\centering
\begin{subfigure}[t]{0.4\textwidth}
\includegraphics[width=\textwidth]{figures/cpi_early_hall_Llama-2-7b-chat-hf.pdf}
\caption{Early-site hallucinations ($\Delta\overline{\text{IE}}(y,u) < 0$)}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
\includegraphics[width=\textwidth]{figures/cpi_late_hall_Llama-2-7b-chat-hf.pdf}
\caption{Late-site hallucinations ($\Delta\overline{\text{IE}}(y,u) \geq 0$)}
\end{subfigure}
\caption{\textbf{Average Indirect Effect (AIE)} of individual model components for (a) early-site (left column) and (b) late-site (right column) non-factual hallucinations. }
\label{fig:cpi-early-late-llama}
\end{figure*}

Following previous work in causal mediation analysis \cite{vig2020investigating,finlayson2021causal,meng2022locating}, we define the \textbf{causal indirect effect} $\text{IE}(z; y, u, \epsilon) = y_{E^*,z} - y_{*}$ of an intermediate hidden representation $z$ as the decrease in the degree of hallucination after mitigating a single hidden state. Averaging over a set of factual queries and a sample of noises for each query, we obtain the average indirect effect (AIE) for each $z$ and its corresponding model component. 


\paragraph{Experiments.}
We collect a set of factual knowledge queries from the ParaRel \cite{elazar-etal-2021-measuring} dataset of cloze-style factual knowledge queries. Each example in ParaRel contains a knowledge tuple $t_c = (s, r, o_c)$ and a prompt generated from hand-curated templates. We evaluated three widely used pretrained LMs with different layouts: 1)  Llama-2-7B-chat (32 layers, 7B parameters, fine-tuned on instruction following) \cite{touvron2023llama}, 2) GPT-J (28 layers, 6B parameters) \cite{gpt-j}, and 3) GPT-2-XL (48 layers, 1.5B parameters) \cite{radford2019language}. For each prompt $u$, we compute the LM predicted conditional probability $p(o|E(u))$ of the next token continuation, where $o$ is taken from the collection of all capitalized alphabetical tokens in the model vocabulary. To resolve the ambiguity issue where a query may allow multiple correct answers, we define hallucinations as the cases where the LM assigns the highest probability to a token $o'$ that is neither the suffix of the true object $o_c$ nor the suffix of any other objects of the subject-relation pair $(s,r)$ returned by a WikiData API query search.  \footnote{See Appendix \ref{appendix:data} for more details about dataset construction.} 


\paragraph{Results.}
We compute the average causal indirect effect over queries from ParaRel for hidden states $z \in Z$ across various sentence positions and transformer layers. Figure \ref{fig:cpi-modules-Llama} shows the AIE distributions for three model components of Llama-2-7B: the residual stream, the attention heads, and the MLPs. We observe two groups of hidden states yielding the highest attribution scores towards incorrectly predicted objects: 1) the hidden states of the subject tokens at lower transformer layers by MLPs, and 2) the hidden states of the last relation token at upper transformer layers by MLPs and attention heads. We observe similar causal effect distributional patterns for GPT models as well (see Appendix \ref{appendix:gpt-cpi-results} for additional results). \citet{geva2023dissecting} recently show that lower layer MLPs and upper layer attention heads are two most crucial LM components for successful factual knowledge recalling. Our causal tracing results not only confirm their finding from a contrapositive perspective, but also reveal an additional component (upper layer MLPs) as an important source of hallucinations. 
% Our causal tracing results therefore offer contrapositive support to the existence of the two-stage fact recalling pipeline discovered by \citet{geva2023dissecting}, by showing that failures of the same two module groups are most likely causing factual errors. 

\paragraph{Early- vs. late-site hallucination.}
Based on the findings above, we hypothesize that there are two different ``mechanisms'' that may cause non-factual hallucinations, as illustrated in Figure \ref{fig:early-late-hall-illustrate}: 1) the LM fails to retrieve correct information about the subject from lower layer components, and 2) the LM successfully retrieves some subject attributes from lower layer components, but the upper layer components fail to distinguish the correct object(s) among retrieved ones. In particular, let $L$ be the number of transformer layers of an LM, we define \textit{early-site components} as attention heads and MLPs located in the first half of LM's layers ($1 \leq l \leq \frac{L}{2}$), and \textit{late-site components} as those located in the second half of LM's layers ($\frac{L}{2} < l \leq L$). We then define the \textbf{relative indirect effect} between intermediate representations by early- and late-site model components as: 

\begin{small}
\begin{align}
    &\Delta \overline{\text{IE}}(y,u)= \textcolor{blue}{\overline{\text{IE}}_\text{late}(y,u)} - \textcolor{red}{\overline{\text{IE}}_\text{early}(y,u)}   \\
    &= \frac{2}{L}\Big[ \textcolor{blue}{\sum_{l=1+\frac{L}{2}}^{L}\overline{\text{IE}}(z^{(l)}_T, y, u)} - \textcolor{red}{\sum_{l=1}^{\frac{L}{2}}\overline{\text{IE}}(z^{(l)}_0, y, u)}\Big], \label{eq:rel-ie}
\end{align} 
\end{small}

\noindent where $\color{red}{\overline{\text{IE}}_\text{early}(y,u)}$ is the average indirect effect of early-site intermediate representations of the first subject token $w_0$ (hidden states in blue dashed boxes in Figure \ref{fig:cpi-modules-Llama}), and $\color{blue}{\overline{\text{IE}}_\text{late}(y,u)}$ is the average indirect effect of late-site intermediate representations of the last relation token $w_T$ of $u$ (hidden states in red dashed boxes in Figure \ref{fig:cpi-modules-Llama}). We categorize a hallucination $(u,o,o')$ as \textbf{early-site} if its lower layer hidden representations have stronger AIEs (i.e. $\Delta \overline{\text{IE}}(y,u)< 0$), and otherwise categorize it as \textbf{late-site} (i.e. $\Delta \overline{\text{IE}}(y,u) \geq 0$). We found that early-site and late-site hallucinations have very different AIE distributions: as shown in \ref{fig:cpi-early-late-llama}, while most components that contribute significantly to early-site hallucinations are located in lower layers when processing subject tokens, late-site hallucinations are mostly caused by components concentrated in upper layers when processing the relation tokens.  

\begin{table}[]
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{1}{c}{Statistics} & Early-site hall. & Late-site hall. \\ \midrule
Amount                            &       (1945 / 31.9\%)      &     (4152 / 68.1\%)       \\
$s$-$o$ assoc.                            &    0.40         &     0.88       \\
$s$-$o'$ assoc.                           &    0.85         &    2.03        \\
Robustness                 &     0.78        &    0.51        \\
Uncertainty                   &     4.39        &    4.17        \\ \bottomrule
\end{tabular}%
}
\caption{External data and Llama-2-7b prediction features for two types of non-factual hallucination.}
\label{tab:hall-mech-manifest-llama}
\end{table}


\paragraph{External manifestations of hallucination mechanisms.} 
To verify that our categorization of hallucinations is not a fabricated dichotomy based solely on internal computation patterns, we next investigate whether there are any external features that can be leveraged to distinguish the two types of hallucinations. We consider the following features of query data and model predictions: the \textbf{subject-object association strength} is measured as the inner product between the input layer embeddings of a subject $s$ and a true object $o$ or a hallucinating object $o'$; the \textbf{robustness} of a predicted object $o'$ is measured as the percentage of Gaussian noise injected during the mitigation run in section \ref{subsec:cpi} which, after being added to the input embeddings, fails to make the model prefer the true answer $o$ over $o'$ (i.e., $y_* < 0 < y$); the \textbf{uncertainty} of model prediction is measured by the entropy of the conditional next-token distribution $p(o|u)$. Table \ref{tab:hall-mech-manifest-llama} summarizes the external measurements. We found that 1) subjects of late-site hallucinations (e.g., \textit{Toulouse}) often have hallucinating objects (e.g., \textit{Paris}) of much stronger association strengths than true objects (e.g., \textit{Bologna}), so that the model fail to ``offset'' the prior propensity of model predicting $o'$ upon seeing $s$. Subjects of early-site hallucinations (e.g., \textit{Orica}), on the other hand, often have much weaker associations with both true (e.g., \textit{Australia}) and hallucinating (e.g., \textit{January}) objects; 2) late-site hallucinations are significantly less robust under input perturbations, probably because the model has already retrieved the correct object from early layers and is just ``one step away'' from distinguishing it; 3) the model is less certain about its predictions when generating early-site hallucinations, a pattern that is consistent with previous findings that epistemic hallucinations are often associated with high predictive uncertainty \cite{xiao-wang-2021-hallucination}. 


\begin{figure}[]
\centering
\includegraphics[width=0.9\columnwidth]{figures/Llama-2-7b-chat-hf-esp.pdf}
\caption{Average dot product between true object embedding and intermediate hidden representations by components of Llama-2-7b in each layer.} 
\label{fig:llama-esp}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%
\subsection{Inspection via embedding space projection} \label{subsec:esp}
In this section, we provide further evidence of the mechanistic difference between early- and late-site hallucinations by looking at the information that each model component writes into the residual stream during inference. 

\paragraph{Method.}
% To analyze what is encoded in a representation ht`, we cast it as a distribution pt` over the vocabulary (Geva et al., 2022bFVZ; Nostalgebraist, 2020), using the same projection applied to final-layer representations (Eq. 2).
As Section \ref{sec:background} suggests, each attention or MLP module at layer $l$ contributes to the model prediction by adding its output hidden state into the embeddings $h^{(l-1)}_i$ produced by the previous layer. Recent work shows that the encoded knowledge of a module can be interpreted by applying the final-layer language model head projection (i.e. dot product) to its intermediate output hidden state, thereby obtaining a distribution over the vocabulary \cite{geva-etal-2022-transformer,dar2023analyzing}. For each example of model hallucination $(u,o,o')$, we use this method by first extracting the intermediate outputs $z \in A \bigcup M$ of all MLPs and attention modules, and then taking the dot product $\Tilde{p}(z,o) = z^Te_{o}$ between $z$ and the row vectors corresponding to $o$ in the final projection layer. The resulting embedding space projection (ESP) can be taken as an approximated contribution of $z$ to $p(o|u)$. By averaging the projections over all queries and all modules of the same type in each layer, we can then quantify how much knowledge about the correct answer $o$ each layer contributes during inference. 

\paragraph{Results.}
We compute the layerwise MLP and attention projections for the true objects averaged over three groups of queries: 1) factual answers (i.e. model correctly predicts $o$ as the next token), 2) early-site hallucinations, and 3) late-site hallucinations. Figure \ref{fig:llama-esp} shows the results. We notice that 1) only lower layer MLPs write information about the true answer into the residual stream, and importantly, the contributions of lower layer MLPs are similar for late-site hallucinations and correctly answered queries, while being much less when the model generates early-site hallucinations. 2) For both types of hallucination, the self-attention components, particularly those in upper layers, write significantly less useful information compared to factually correct answers. Similar patterns observed in GPT models can be found in Appendix \ref{appendix:gpt-esp-results}. 

Taken together, our analysis suggests that 1) \textit{early-site MLPs, late-site self-attentions and late-site MLPs are the most crucial LM components of causing hallucinations}, and 2) \textit{lower layer MLPs and upper layer attentions/MLPs do not always break down simultaneously, thus leading to two distinct mechanisms of LM factual errors.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
